Competition Dynamics Shape Algorithmic Phases of In-Context Learning

In-Context Learning (ICL) has significantly expanded the general-purpose nature of large language models, allowing them to adapt to novel tasks using merely the inputted context. This has motivated a series of papers that analyze tractable synthetic domains and postulate precise mechanisms that may underlie ICL. However, the use of relatively distinct setups that often lack a sequence modeling nature to them makes it unclear how general the reported insights from such studies are. Motivated by this, we propose a synthetic sequence modeling task that involves learning to simulate a finite mixture of Markov chains. As we show, models trained on this task reproduce most well-known results on ICL, hence offering a unified setting for studying the concept. Building on this setup, we demonstrate we can explain a model's behavior by decomposing it into four broad algorithms that combine a fuzzy retrieval vs. inference approach with either unigram or bigram statistics of the context. These algorithms engage in a competition dynamics to dominate model behavior, with the precise experimental conditions dictating which algorithm ends up superseding others: e.g., we find merely varying context size or amount of training yields (at times sharp) transitions between which algorithm dictates the model behavior, revealing a mechanism that explains the transient nature of ICL. In this sense, we argue ICL is best thought of as a mixture of different algorithms, each with its own peculiarities, instead of a monolithic capability. This also implies that making general claims about ICL that hold universally across all settings may be infeasible.

==> trash/past_text.tex <==

\textbf{ESL notes.} Repeating contributions as per meeting. We should get on the same page about results (or hypotheses if things are not settled yet) and narrative / story first, dividing work from there. Given we have a superset of results from the other project too, converging on the story will help reuse relevant results and code.
\begin{itemize}
    \item Emergence w.r.t.\ model scale.(FLOPs in main figure, n-steps and network width separately in appendix)
    \item Emergence w.r.t.\ data diversity.
    \item Implicating change of mechanism in emergence: retrieval to inference of bigram statistics
    \item What else?
\end{itemize}
\core{What if we organized as below, where we first introduce the phenomena, mechanistically analyze it then go to scaling law. The motivation is as follows. There are multiple ways one might see a sudden gain/improvement in accuracy/loss, I think there could also be less interesting modes of non-linear evolution. So lets first get the readers 100\% on board that there is a mechanism change and not just ``some empirical gain".}
\begin{enumerate}
    \item Introduction
    \item Theory \& Setup
    \begin{enumerate}
        \item Setup
        \item Bayesian Solution and theoretical scaling prediction
        \item Proposition of further division of in-context task learning
        \todo{ESL: Note to self. Read the two modes of ICL paper.}
    \end{enumerate}
    \item Results
    \begin{enumerate}
        \item Emergence w.r.t.\ data diversity
        \begin{itemize}
            \item Make a K vs.\ N phase diagram?
        \end{itemize}
        \item Mechanistic Analysis: retrieval to inference of bigram statistics
        \item Emergence w.r.t.\ model scale \& Phase diagrams
        \begin{itemize}
            \item What control variables for phase diagram?
        \end{itemize}
        \item Emergence w.r.t.\ context size \core{results not here yet}
        \item Basis transitions and compositional generalization \core{Definitely post-submission}
        \item Theoretically trying to justify results
    \end{enumerate}
    \item Discussion\&Related Works
    \begin{enumerate}
        \item Bayesian Prior Relaxation \core{The process can be understood as a relaxation of the prior space from certain markov transitions to ``all" markov transitions.}
        \item Compositional Generalization \core{The above suggests a possible geometry of generalization in task space. One can think of compositional generalization as generalizing to the tail of distributions.}
        \item Types of in-context learning.
        \item Implication to Emergent Phenomena
        \item Intuition on inference temperature
        \item Comparison with Edelman et al. 2023
    \end{enumerate}
\end{enumerate}
